Exploring Indoor Health: An In-depth Field Study on the Indoor Air Quality Dynamics

Indoor air pollution, a significant driver of respiratory and cardiovascular diseases, claims 3.2 million lives yearly, according to the World Health Organization, highlighting the pressing need to address this global crisis. In contrast to unconstrained outdoor environments, room structures, floor plans, ventilation systems, and occupant activities all impact the accumulation and spread of pollutants. Yet, comprehensive in-the-wild empirical studies exploring these unique indoor air pollution patterns and scope are lacking. To address this, we conducted a three-month-long field study involving over 28 indoor spaces to delve into the complexities of indoor air pollution. Our study was conducted using our custom-built DALTON air quality sensor and monitoring system, an innovative IoT air quality monitoring solution that considers cost, sensor type, accuracy, network connectivity, power, and usability. Our study also revealed that conventional measures, such as the Indoor Air Quality Index (IAQI), don't fully capture complex indoor air quality dynamics. Hence, we proposed the Healthy Home Index (HHI), a new metric considering the context and household activities, offering a more comprehensive understanding of indoor air quality. Our findings suggest that HHI provides a more accurate air quality assessment, underscoring the potential for wide-scale deployment of our indoor air quality monitoring platform.

==> Sections/acknowledge.tex <==
\section{Acknowledgement}

==> Sections/discuss.tex <==
\section{Limitations \& Future Work}
to be written.

==> Sections/method.tex <==
%\section{Methodology}
%
%%\subsection{Designing a new metric}
%%- based on effects on health and exposure time for each pollutants.\\
%%- Must be scaled within 0-100 or finite categories \\
%%- Proof of upper bound or insight of each category\\
%%- Consider all major pollutants \\
%
%\subsection{Feature Engineering}
%set of features and cross-modal filtering/ imputation for missing data.
%
%
%
%\subsection{Joint-Optimization of Placement \& Metric Estimation}
%\subsubsection{Sensor Placement Strategy}
%\paragraph{Static Placement}
%sensor positions for each house is fixed throughout the day
%\paragraph{Dynamic Placement}
%sensor positions change over the course of day to better capture temporal pollution sources
%
%\subsubsection{Model}


==> Sections/platform.tex <==
\section{\ourmethod{} Platform}
\label{sec:platform}
In this section, we discuss the details of our in-house sensing module and the underline IoT infrastructure that enables real-time data streaming, storage, data analytics, and fault recovery mechanism to facilitate a plug-and-play user experience. As shown in \figurename~\ref{fig:sensors}, one can realize the sensing module as a lunchbox size (112 mm $\times$ 112 mm $\times$ 55 mm) device. The detail follows. 


%The module can be placed at any corner of the house, having a standard wall socket to provide power and a WiFi router within the connectivity. For example, study table, bedside table, living room, kitchen, etc., are some locations where one can place the module to estimate daily pollution exposure. After an initial setup, the module automatically connects to the house's WiFi and sends data to the IoT backbone. Upon receiving multiple such parallel data streams from the sensing modules deployed across several indoor environments, the IoT backbone segregates the streams and stores in a NoSQL database, exposing endpoints for real-time data analytics and fault recovery. The specifications of the sensing module and the workflow of the IoT backbone is explained as follows.



%With increasing adaption of smart home devices like Amazon Alexa~\cite{}, Google Home~\cite{}, Wi-Fi connection have become ubiquitous. The sensing module has a similar footprint as such smart home devices in terms of size and

\subsection{In-house Sensing Module}
\label{sec:sensing_module}
We designed the in-house sensing module shown in \figurename~\ref{fig:sensors}, considering its seamless integration with today's indoor environments. The device is equipped with WiFi 2.4GHz HT40 capabilities to connect to the IoT backbone. The backbone handles the data stream from the module, which samples the environment at a scan rate of $1$ Hz. An external 5V DC adapter powers the sensing module and it draws a maximum 300mA current, displacing at most 1.5W. \tablename~\ref{tab:ovl_spec} details the module's system specification and operational bounds.

The primary building blocks of the module can be segregated into three groups. \textit{First}, the outer shell of the module is a 3D printed (PLA+ material) hollow structure that has three sub-components (i) the lead, (ii) the side-walls, and (ii) the bottom-stand, which is screwed together to provide physical damage protection. We design the outer shell with honeycomb holes so that the air within the module is the same as outside, resulting in unbiased measurement of pollutants. \textit{Secondly}, the processing unit and the connectivity board export multiple input sockets to connect respective sensors. We utilize the ESP-WROOM-32 chip as the on-device processing unit that packs a dual-core Xtensa 32-bit LX6 MCU with WiFi capabilities. The connectivity board is a two-layer printed circuit board (FR4 material). \textit{Thirdly}, the device is equipped with multiple research-grade sensors that together measure concentration of pollutants, such as \textit{Particulate matter} (PM\textsubscript{x}), \textit{Nitrogen dioxide} (NO\textsubscript{2}), \textit{Ethanol} (C\textsubscript{2}H\textsubscript{5}OH), \textit{Vola\textit{tile organic compounds} (VOCs), \textit{Carbon monoxide} (CO), }Carbon dioxide (CO\textsubscript{2}), etc., with \textit{Temperature} (T) and \textit{Relative humidity} (RH).

%list of pollutants, measuring ranges and error margins.
%Assambly, and data streaming backbone MQTT.

\subsection{IoT Backbone}
To handle multiple real-time data streams from a large set of sensing modules deployed across several households, we design the IoT backbone (shown in \figurename~\ref{fig:backend}) with multiple modular micro-services individually responsible for singular tasks. The benefit of such a micro-service architecture is that it allows real-time data analytics and stream processing, which reduces the possibility of single points of failure. Below are the design choices and micro-services of the IoT backbone.
\begin{figure}[!ht]
	\centering
	\includegraphics[width=0.95\columnwidth]{Figures/Diagrams/backend.pdf}
	\caption{IoT Backbone Architecture}
	\label{fig:backend}
\end{figure}

\subsubsection{IP Agnostic Design}
In real-world, large-scale IoT sensing networks with multiple local area networks, the public IP addresses of each module are not always accessible because of restrictions imposed by ISPs and limited expertise by end users. We chose a publisher-subscriber-based IP agnostic approach (through a micro-service described in the next subsection) where any sensing module can be uniquely identified. In addition, sensing modules and micro-services of the IoT backbone can establish an asynchronous communication channel. The design simplifies the initial setup for the end user and allows supervisory control over each module, allowing remote debugging, and reconfiguration.

\subsubsection{Micro-services} 
The IoT backbone is comprised of several micro-services as follows. \textbf{ (1) Queuing} service hosts an MQTT broker\footnote{Eclipse Mosquitto (\url{https://mosquitto.org/}) is utilized as the message broker} that manages the DATA queue and the command (CMD) queue as shown in \figurename~\ref{fig:backend} and ensures one-time FIFO delivery in the underline asynchronous wireless channel. The broker's publisher-subscriber interface also allows indirect communication between sensing modules and the rest of the IoT backbone. \textbf{(2) Database} service hosts a MongoDB server that keeps track of four collections, namely data, error log, users, and annotation, to facilitate storage for the corresponding micro-services of the IoT backbone. \textbf{(3) Data Stream Processor} subscribes to the mixed data stream of the queuing service and splits it into individual streams from each sensing module. In addition, it checks the data for basic anomalies (continuous zeros or maximums) and stores the valid data. \textbf{(4) Command Pusher} exposes endpoints for remotely executing commands such as reboot, reset, reconfiguration, etc., in the sensing modules. \textbf{(5) Fault Recovery} is triggered by the stream processor upon detecting any anomaly in the streaming sensor data. The fault recovery service determines the type of fault and the suitable recovery action (i.e., reboot) for the specific device. Consequently, it stores the error log in the error log collection of the database service and queries the Command Pusher to schedule the recovery action. \textbf{(6) Annotation} service exposes secured endpoints for tagging indoor activities for each occupant via a simple android application named \textit{VocalAnnot} (details in Section~\ref{sec:datacollection}). The annotation service receives timestamped ground truth activity labels and stores them in the database. \textbf{(7) Admin Portal} with a role-based access control provides an interface for executing commands remotely, listing live modules that are sending data, viewing error log, and recovery actions to debug any infrastructural or hardware issues (i.e., unstable power supply, damaged sensor), plot live data, etc. 

In summary, \ourmethod{} is a very extensible IoT platform comprised of an  in-house sensing module and a robust IoT backbone to facilitate plug-and-play end-user experience. Next, we describe the field study with the developed platform for data collection.


% \begin{enumerate}
% 	\item \textbf{Queuing} service hosts a MQTT broker\footnote{Eclipse Mosquitto (\url{https://mosquitto.org/}) is utilized as the message broker} that manages the DATA queue and the CMD queue as shown in \figurename~\ref{fig:backend}. Queuing of the data, and control signals are necessary to ensure FIFO and one-time-delivery in the underline asynchronous wireless channel utilized by the sensing modules. Moreover, the queuing service allows both-way indirect communication among sensing modules and the rest of the IoT backbone over the publisher-subscriber interface of the broker. 
	
% 	\item \textbf{Database} service hosts a MongoDB server that keeps track of four collection namely data, errorlog, users, annot to facilitated storage for the corresponding micro-services of the IoT backbone.  
	
% 	\item \textbf{Data Stream Processor} subscribes to the mixed data stream of the queuing service and split it into individual streams from each sensing module. Moreover, it performs basic sanity checks in the streaming data to detect faulty sensor values in the data item from each of the sensing module. Upon detecting such anomaly for any sensing module, the stream processor fallback to the fault recovery service for that specific module. Meanwhile data items that pass the sanity check are then stored in the data collection of the database service.
	
% 	\item \textbf{Command Pusher} exposes endpoints for remotely executing commands such as reboot, reset, reconfiguration etc., in the sensing modules. Upon querying a specific endpoint along with the affected device ID, the Command Pusher keeps a log of the event and encode the command to a format that is understandable by the sensing modules. Further it publish the encoded command to the CMD queue, which is then reliably broadcasted to all sensing modules via the asynchronous communication channel. At the device end, only desired recipients of the command decode and execute further while other simply drop it.
	
% 	\item \textbf{Fault Recovery} is triggered by the stream processor upon detecting any anomaly in the streaming sensor data. The fault recovery service determine the type of fault and suitable recovery action (i.e., reboot) for the specific device. Consequently, it stores the error log in errorlog collection of the database service and query the Command Pusher to schedule the recovery action.
	
% 	\item \textbf{Annotation} service exposes secured endpoints for tagging indoor activities for each occupant via a simple android application named VocalAnnot. The annotation service receives timestamped ground truth activity labels and stores them in the annot collection of the database service. Details on the VocalAnnot app is further described in Section~\ref{sec:datacollection}.
	
% 	\item \textbf{Admin Portal} provides an elegant interface for executing commands remotely, list live modules that are sending data, view errorlog and recovery actions to debug any infrastructural or hardware issues (i.e., unstable power supply, damaged sensor), plot live data, etc. Moreover, the portal provides role-based access control such that end-users have limited capabilities to change configuration of the IoT framework, where admins can alter every aspect of the same.
	
% \end{enumerate}



  
